Numerical Solution of Initial Value Problems

Welcome to a beautiful subject in scientific computing: numerical solution of ordinary differential equations (ODEs) with initial conditions.

==> workouts_3.tex <==

\section{Additional workouts}









